Modelling of Flow Past Long Cylindrical Structures

Turbulent flows are fundamental in engineering and the environment, but their chaotic and three-dimensional (3-D) nature makes them computationally expensive to simulate. In this work, a dimensionality reduction technique is investigated to exploit flows presenting an homogeneous direction, such as wake flows of extruded two-dimensional (2-D) geometries. First, we examine the effect of the homogeneous direction span on the wake turbulence dynamics of incompressible flow past a circular cylinder at $Re=10^4$. It is found that the presence of a solid wall induces 3-D structures even in highly constricted domains. The 3-D structures are rapidly two-dimensionalised by the large-scale K\'{a}rm\'{a}n vortices if the cylinder span is 50\% of the diameter or less, as a result of the span being shorter than the natural wake Mode B instability wavelength[...]. With this physical understanding, a 2-D data-driven model that incorporates 3-D effects, as found in the 3-D wake flow, is presented. The 2-D model is derived from a novel flow decomposition based on a local spanwise average of the flow, yielding the spanwise-averaged Navier-Stokes (SANS) equations[...]. A machine-learning (ML) model is employed to provide closure to the SANS equations. In the a-priori framework, the ML model yields accurate predictions of the SSR terms, in contrast to a standard eddy-viscosity model which completely fails to capture the closure term structures[...]. In the a-posteriori analysis, while we find evidence of known stability issues with long-time ML predictions for dynamical systems, the closed SANS equations are still capable of predicting wake metrics and induced forces with errors from 1-10%. This results in approximately an order of magnitude improvement over standard 2-D simulations while reducing the computational cost of 3-D simulations by 99.5%.

==> chapters/nomenclature.tex <==
\chapter{Nomenclature}
\markboth{NOMENCLATURE}{}

\textbf{{\large Upper-case Roman}}

\begin{longtable}[l]{ll}
$\mathcal{B}$ & Solid body governing equation\tabularnewline
$C_D$ & Drag coefficient\tabularnewline
$C_L$ & Lift coefficient\tabularnewline
$C_s$ & Smagorinsky model constant\tabularnewline
$\mathcal{CC}$ & Correlation coefficient\tabularnewline
$D$ & Cylinder diameter\tabularnewline
$E$ & Kinetic energy \tabularnewline
$\mathcal{F}$ & Fluid governing equation\tabularnewline
$F_x$ & Drag force\tabularnewline
$F_y$ & Lift force\tabularnewline
$H$ & Helicity \tabularnewline
$II, III$ & Non-zero invariants of the anisotropic Reynolds-stress tensor \tabularnewline
$K_\epsilon$ & BDIM convolution kernel \tabularnewline
$L$ & Characteristic length\tabularnewline
$L_{11}$ & Integral lengthscale\tabularnewline
$L_a$ & Spanwise-averaging length\tabularnewline
$L_z$ & Cylinder span\tabularnewline
$M$ & Number of time steps\tabularnewline
$\mathcal{M}$ & Meta-equation combining fluid and solid governing equations\tabularnewline
$N$ & Number of grid points\tabularnewline
$P$ & Spanwise-averaged pressure\tabularnewline
$R$ & Ratio of mean vortex-stretching term to mean vortex-advection term\tabularnewline
$Re$ & Reynolds number \tabularnewline
$\mathcal{S}$ & 3-D Navier--Stokes spatial operator \tabularnewline
$\tilde{\mathcal{S}}$ & 2-D Navier--Stokes spatial operator \tabularnewline
$\mathcal{S}^R$ & Perfect closure \tabularnewline
$S_{ij}$ & Rate-of-strain tensor \tabularnewline
$St$ & Strouhal number \tabularnewline
$\vect{U}$ & Spanwise-averaged velocity vector field \tabularnewline
$U$ & Characteristic velocity\tabularnewline
$U$ & Spanwise-averaged velocity component along the $x$ spatial direction\tabularnewline
$U_\infty$ & Free-stream velocity\tabularnewline
$V$ & Spanwise-averaged velocity component along the $y$ spatial direction\tabularnewline
$W$ & Spanwise-averaged velocity component along the $z$ spatial direction\tabularnewline
$\mathrm{X}_n$ & Model input set\tabularnewline
$\mathrm{Y}_n$ & Model output set\tabularnewline
$Z$ & Enstrophy \tabularnewline
\end{longtable}

\textbf{{\large Lower-case Roman}}

\begin{longtable}[l]{ll}
$b_{ij}$ & Anisotropic Reynolds-stress tensor \tabularnewline
$d$ & Distance function\tabularnewline
$f_s$ & Vortex-shedding frequency \tabularnewline
$\vect{h}$ & Force vector field combining convective and viscous forces\tabularnewline
$k$ & Turbulence kinetic energy \tabularnewline
$p$ & Pressure field \tabularnewline
$\vect{r}$ & Distance vector\tabularnewline
$r$ & Radial direction in the cylindrical coordinates frame\tabularnewline
$t$ & Time\tabularnewline
$t^*$ & Convective time ($t$ scaled with $U$ and $L$)\tabularnewline
$\vect{u}$ & Velocity vector field\tabularnewline
$u$ & Velocity component along the $x$ spatial direction\tabularnewline
$\vect{u}_b$ & Velocity boundary condition on solid walls\tabularnewline
$\vect{u}_s$ & Straining velocity vector field\tabularnewline
$\vect{u}_v$ & Columnar vortex velocity vector field\tabularnewline
$v$ & Velocity component along the $y$ spatial direction\tabularnewline
$w$ & Velocity component along the $z$ spatial direction\tabularnewline
$\vect{x}$ & Spatial coordinates vector \tabularnewline
$x$ & Spatial coordinate aligned with the principal (streamwise) flow direction\tabularnewline
$y$ & Spatial coordinate aligned with the transverse (crossflow) flow direction\tabularnewline
$z$ & Spatial coordinate aligned with the lateral (spanwise) flow direction\tabularnewline
\end{longtable}

\textbf{{\large Upper-case Greek}}

\begin{longtable}[l]{ll}
$\Gamma$ & Circulation\tabularnewline
$\Delta$ & LES filter size\tabularnewline
$\vect{\Omega}$ & Spanwise-averaged vorticity vector field \tabularnewline
$\Omega$ & A general spatial domain \tabularnewline
$\Omega_f$ & Fluid subdomain \tabularnewline
$\Omega_b$ & Solid body subdomain \tabularnewline
\end{longtable}

\textbf{{\large Lower-case Greek}}

\begin{longtable}[l]{ll}
$\gamma$ & Rate of strain\tabularnewline
$\delta_{ij}$ & Kronecker delta tensor \tabularnewline
$\delta t$ & Temporal resolution\tabularnewline
$\delta x$ & Spatial resolution\tabularnewline
$\delta_\epsilon$ & Zeroth-moment of the BDIM convolution kernel \tabularnewline
$\epsilon$ & Turbulence dissipation rate \tabularnewline
$\epsilon_T$ & Trapezoidal quadrature error \tabularnewline
$\vect{\zeta}^R$ & Spanwise-stress residual vector in the spanwise-averaged VTE \tabularnewline
$\eta$ & Invariant of the anisotropic Reynolds-stress tensor \tabularnewline
$\eta$ & Kolmogorov lengthscale \tabularnewline
$\theta$ & Angular direction in the cylindrical coordinates frame\tabularnewline
$\theta_l$ & Lower separation angle on the cylinder surface\tabularnewline
$\theta_u$ & Upper separation angle on the cylinder surface\tabularnewline
$\vect{\kappa}$ & Wavenumber vector\tabularnewline
$\kappa$ & Wavenumber\tabularnewline
$\lambda_z$ & Spanwise correlation length \tabularnewline
$\mu$ & Dynamic viscosity\tabularnewline
$\nu$ & Kinematic viscosity\tabularnewline
$\nu_{e}$ & Effective kinematic eddy viscosity in iLES\tabularnewline
$\nu_{t}$ & Kinematic eddy viscosity\tabularnewline
$\xi$ & Invariant of the anisotropic Reynolds-stress tensor \tabularnewline
$\rho$ & Density\tabularnewline
$\sigma$ & Standard deviation\tabularnewline
$\tau$ & Turbulence timescale\tabularnewline
$\vect{\tau}_{ij}^R$ & Spanwise-stress residual tensor\tabularnewline
$\vect{\tau}_{ij}^r$ & Anisotropic spanwise-stress residual tensor\tabularnewline
$\chi_{12}$ & Two-point correlation function\tabularnewline
$\vect{\omega}$ & Vorticity vector field\tabularnewline
$\vect{\omega}_v$ & Columnar vortex vorticity vector field\tabularnewline
\end{longtable}

\textbf{{\large Acronyms}}

\begin{longtable}[l]{ll}
2-D & Two-Dimensional\tabularnewline
3-D & Three-Dimensional\tabularnewline
ANN & Artificial Neural Network \tabularnewline
BDIM & Boundary Data Immersion Method \tabularnewline
CNN & Convolutional Neural Network \tabularnewline
DNS & Direct Numerical Simulation \tabularnewline
EVM & Eddy-Viscosity Model \tabularnewline
FLOP & FLoating-point OPerations\tabularnewline
FSI & Fluid-Structure Interaction\tabularnewline
HPC & High-Performance Computing \tabularnewline
IB & Immersed Boundary\tabularnewline
iLES & implicit Large-Eddy Simulation\tabularnewline
KLB & Kraichnan--Leith--Batchelor\tabularnewline
LES & Large-Eddy Simulation\tabularnewline
ML & Machine-Learning\tabularnewline
MIMO & Multiple-Input Multiple-Output \tabularnewline
PBML & Physics-Based Machine Learning\tabularnewline
PS & Power Spectrum\tabularnewline
QUICK & Quadratic Upstream Interpolation for Convective Kinematics\tabularnewline
RANS & Reynolds-Averaged Navier--Stokes\tabularnewline
ReLU & Rectified Linear Unit \tabularnewline
RNN & Recurrent Neural Network \tabularnewline
SANS & Spanwise-Averaged Navier--Stokes\tabularnewline
SGS & SubGrid Scale\tabularnewline
SSR & Spanwise-Stress Residual\tabularnewline
TKE & Turbulence Kinetic Energy\tabularnewline
VIV & Vortex-Induced Vibrations\tabularnewline
VTE & Vorticity Transport Equation\tabularnewline
\end{longtable}
